OPT-IML: Scaling Language Model Instruction Meta Learning through the Lens of Generalization

Recent work has shown that fine-tuning large pre-trained language models on a collection of tasks described via instructions, a.k.a. instruction-tuning, improves their zero and few-shot generalization to unseen tasks. However, there is a limited understanding of the performance trade-offs of different decisions made during the instruction-tuning process. These decisions include the scale and diversity of the instruction-tuning benchmark, different task sampling strategies, fine-tuning with and without demonstrations, training using specialized datasets for reasoning and dialogue, and finally, the fine-tuning objectives themselves. In this paper, we characterize the effect of instruction-tuning decisions on downstream task performance when scaling both model and benchmark sizes. To this end, we create OPT-IML Bench: a large benchmark for Instruction Meta-Learning (IML) of 2000 NLP tasks consolidated into task categories from 8 existing benchmarks, and prepare an evaluation framework to measure three types of model generalizations: to tasks from fully held-out categories, to held-out tasks from seen categories, and to held-out instances from seen tasks. Through the lens of this framework, we first present insights about instruction-tuning decisions as applied to OPT-30B and further exploit these insights to train OPT-IML 30B and 175B, which are instruction-tuned versions of OPT. OPT-IML demonstrates all three generalization abilities at both scales on four different evaluation benchmarks with diverse tasks and input formats -- PromptSource, FLAN, Super-NaturalInstructions, and UnifiedSKG. Not only does it significantly outperform OPT on all benchmarks but is also highly competitive with existing models fine-tuned on each specific benchmark. We release OPT-IML at both scales, together with the OPT-IML Bench evaluation framework.

==> opt_comparison.tex <==
\begin{table}[]
\begin{tabular}{l|l|lllll|lllll}
\toprule
              &            & \multicolumn{5}{c|}{OPT}      & \multicolumn{5}{c}{\Ours}      \\ \hline
              & Eval Split & 1.3B & 13B & 30B & 66B & 175B & 1.3B & 13B & 30B & 66B & 175B \\ \hline
HellaSwag     &            &      &     &     &     &      &      &     &     &     &      \\
StoryCloze    &            &      &     &     &     &      &      &     &     &     &      \\
PIQA          &            &      &     &     &     &      &      &     &     &     &      \\
Arc Easy      &            &      &     &     &     &      &      &     &     &     &      \\
Arc Challenge &            &      &     &     &     &      &      &     &     &     &      \\
OpenBookQA    &            &      &     &     &     &      &      &     &     &     &      \\
Winograd      &            &      &     &     &     &      &      &     &     &     &      \\
Winogrande    &            &      &     &     &     &      &      &     &     &     &      \\
MultiRC       &            &      &     &     &     &      &      &     &     &     &      \\
Record        &            &      &     &     &     &      &      &     &     &     &      \\
WiC           &            &      &     &     &     &      &      &     &     &     &      \\
BoolQ         &            &      &     &     &     &      &      &     &     &     &      \\
RTE           &            &      &     &     &     &      &      &     &     &     &      \\
COPA          &            &      &     &     &     &      &      &     &     &     &      \\
CB            &            &      &     &     &     &      &      &     &     &     &      \\
WSC           &            &      &     &     &     &      &      &     &     &     &      \\
\bottomrule
\end{tabular}
\caption{0-shot accuracy evaluations on the 16 tasks reported by OPT \citep{zhang2022opt}. \Ours improves over OPT on X out of Y tasks despite not having seen these tasks during fine-tuning. Note that COPA was part of our validation set and was used for early-stopping and hyper-parameter tuning. PIQA, Arc Easy/Challenge, OpenBookQA, MultiRC, Record, and BoolQ came from partially held-out evaluation clusters i.e. \Ours has seen other tasks belonging to the same cluster as these tasks. The remaining tasks are completely held-out i.e. all other tasks in the same cluster are also held out.}
\label{tab:optzero}
\end{table}

\begin{table}[]
\begin{tabular}{l|l|lllll|lllll}
\toprule
              &            & \multicolumn{5}{c|}{OPT}      & \multicolumn{5}{c}{\Ours}      \\ \hline
              & Eval Split & 1.3B & 13B & 30B & 66B & 175B & 1.3B & 13B & 30B & 66B & 175B \\ \hline
HellaSwag     &            &      &     &     &     &      &      &     &     &     &      \\
StoryCloze    &            &      &     &     &     &      &      &     &     &     &      \\
PIQA          &            &      &     &     &     &      &      &     &     &     &      \\
Arc Easy      &            &      &     &     &     &      &      &     &     &     &      \\
Arc Challenge &            &      &     &     &     &      &      &     &     &     &      \\
OpenBookQA    &            &      &     &     &     &      &      &     &     &     &      \\
Winograd      &            &      &     &     &     &      &      &     &     &     &      \\
Winogrande    &            &      &     &     &     &      &      &     &     &     &      \\
MultiRC       &            &      &     &     &     &      &      &     &     &     &      \\
Record        &            &      &     &     &     &      &      &     &     &     &      \\
WiC           &            &      &     &     &     &      &      &     &     &     &      \\
BoolQ         &            &      &     &     &     &      &      &     &     &     &      \\
RTE           &            &      &     &     &     &      &      &     &     &     &      \\
COPA          &            &      &     &     &     &      &      &     &     &     &      \\
CB            &            &      &     &     &     &      &      &     &     &     &      \\
WSC           &            &      &     &     &     &      &      &     &     &     &      \\
\bottomrule
\end{tabular}
\caption{Few-shot accuracy evaluations on the 16 tasks reported by OPT \citep{zhang2022opt}. \Ours improves over OPT on X out of Y tasks despite not having seen these tasks during fine-tuning. See the caption in Table \ref{tab:optzero} for more details. }
\label{tab:optfew}
\end{table}

==> table_task_split_details.tex <==
\begin{landscape}
{\small\tabcolsep=3pt
\begin{longtable}{ll|rrrrrrrrr|rrlllll}
    \toprule
    \multirow{2}{*}{Split} & \multirow{2}{*}{Task Family} & \multicolumn{9}{c}{\#\ datasets } & \multirow{2}{*}{\makecell{\#\\exp.}} & \multirow{2}{*}{\makecell{avg. \# promp.\\/dataset}} & \multirow{2}{*}{\makecell{\#\\tokens}} & \multicolumn{4}{c}{prompt length} \\
    & &  NIv2 & PS &  CF &  FL &  EM &  T5 &  US &  BB & All  & & & & min & max & mean & std\outlier \\
    \cmidrule(lr){1-2} \cmidrule(lr){3-11} \cmidrule(lr){12-14} \cmidrule(lr){15-18}
    \endhead
    \multirow{36}{*}{\makecell{Train \\ (94)}}   &                 question answering &             109 &                      63 &                  33 &               8 &                1 &             4 &                      5 &                   0 &              223 &        18.6M &              2.3 &    1980.7M &               4.0 &            121.0K &              369.6 &              1.3K \\
           &                      summarization &              13 &                      11 &                   6 &               9 &                0 &             1 &                      0 &                   0 &               40 &         4.9M &              3.4 &    1083.1M &              10.0 &            645.3K &              684.0 &             888.8 \\
           &                        translation &             393 &                       0 &                   0 &              10 &                0 &             6 &                      0 &                   0 &              409 &         2.8M &              1.2 &     406.1M &               8.0 &             39.6K &              276.9 &             204.6 \\
           &                 sentiment analysis &              65 &                       3 &                  10 &               4 &                0 &             0 &                      0 &                   0 &               82 &         2.3M &              1.4 &     316.5M &               2.0 &             12.0K &              189.5 &             155.9 \\
           &                question generation &              64 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &               64 &       492.6K &              1.0 &     276.2M &              33.0 &            120.9K &              547.2 &              1.6K \\
           &                text categorization &              34 &                       4 &                   4 &               0 &                0 &             0 &                      0 &                   0 &               42 &         2.2M &              1.5 &     253.8M &               3.0 &              4.2K &              220.9 &             175.2 \\
           &                       data to text &               4 &                       4 &                   2 &               1 &                0 &             0 &                      0 &                   0 &               11 &         1.0M &              2.3 &     223.3M &              10.0 &              8.8K &              211.8 &             323.3 \\
           &                  fill in the blank &               7 &                       5 &                   0 &               0 &                0 &             0 &                      0 &                   0 &               12 &       457.8K &              2.7 &     200.0M &              15.0 &              1.9K &              248.9 &             202.9 \\
           &                       UNCLASSIFIED &              38 &                      10 &                  13 &               4 &                0 &             0 &                      0 &                   0 &               65 &         3.1M &              2.4 &     192.6M &               2.0 &              2.1K &              106.7 &             153.3 \\
           &      generated-text classification &               0 &                       0 &                   0 &               0 &                1 &             0 &                      0 &                   0 &                1 &       100.0K &              1.0 &      62.5M &              19.0 &              1.0K &              624.7 &               0.0 \\
           &                  program execution &              90 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &               90 &       433.9K &              1.0 &      57.7M &              36.0 &             646.0 &              129.3 &              50.3 \\
           &            hyperpartisan detection &               0 &                       2 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                2 &       100.6K &              5.5 &      52.3M &              42.0 &              1.3K &              512.2 &               7.9 \\
           &        discourse marker prediction &               0 &                       1 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                1 &       100.0K &              5.0 &      49.4M &              25.0 &             833.0 &              494.2 &               0.0 \\
           &                       text to code &              12 &                       2 &                   0 &               0 &                0 &             0 &                      0 &                   0 &               14 &       149.6K &              1.0 &      47.2M &              56.0 &              1.1K &              509.7 &             212.1 \\
           &              sentence perturbation &              14 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &               14 &       311.4K &              1.0 &      47.1M &              53.0 &              2.9K &              141.0 &              51.3 \\
           &                   semantic parsing &               0 &                      12 &                   0 &               0 &                2 &             0 &                      6 &                   0 &               20 &       322.9K &              5.2 &      45.3M &              13.0 &              1.6K &              181.7 &             266.7 \\
           &           sentiment classification &               0 &                       6 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                6 &       236.0K &              7.5 &      37.7M &               9.0 &              1.1K &              201.2 &             189.2 \\
           &               topic classification &               0 &                       4 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                4 &       301.7K &              5.0 &      35.1M &              11.0 &              1.5K &               98.7 &              48.8 \\
           &                      text matching &              40 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &               40 &       161.4K &              1.0 &      34.5M &              54.0 &              2.3K &              192.4 &             115.1 \\
           &                       paraphrasing &               9 &                       4 &                   4 &               4 &                0 &             0 &                      0 &                   0 &               21 &       715.8K &              3.6 &      34.0M &              10.0 &             405.0 &               88.1 &              44.7 \\
           &                       text scoring &               0 &                      10 &                   0 &               0 &                0 &             0 &                      0 &                   0 &               10 &       436.4K &              3.9 &      27.0M &              12.0 &              7.4K &               74.0 &              54.0 \\
           &                        pos tagging &              10 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &               10 &        62.1K &              1.0 &      25.7M &              51.0 &              2.4K &              410.6 &             174.4 \\
           &          word sense disambiguation &               0 &                       1 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                1 &       100.0K &              3.0 &      25.5M &              26.0 &             689.0 &              255.4 &               0.0 \\
           &             information extraction &              18 &                       1 &                   4 &               0 &                0 &             0 &                      0 &                   0 &               23 &         1.2M &              1.0 &      25.0M &               3.0 &             25.7K &              204.8 &             288.5 \\
           &           toxic language detection &              25 &                       1 &                   3 &               0 &                1 &             0 &                      0 &                   0 &               30 &       244.1K &              1.0 &      23.4M &               3.0 &              3.2K &              122.3 &              56.9 \\
           &         commonsense classification &              23 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &               23 &       130.3K &              1.0 &      23.4M &              67.0 &             242.0 &              174.5 &              36.7 \\
           & semantic similarity classification &               0 &                       6 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                6 &       332.2K &              9.5 &      20.9M &              15.0 &             333.0 &               69.4 &              12.9 \\
           &                  dialogue modeling &               0 &                       4 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                4 &       294.6K &              2.0 &      20.9M &               5.0 &             727.0 &              100.3 &              61.9 \\
           &                   title generation &              15 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &               15 &        55.4K &              1.0 &      19.5M &              33.0 &             22.0K &              421.7 &             353.3 \\
           &       answerability classification &              13 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &               13 &        45.9K &              1.0 &      19.1M &              93.0 &              2.6K &              337.5 &             287.4 \\
           &                       code to text &               4 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                4 &        40.0K &              1.0 &      16.6M &             287.0 &             809.0 &              450.9 &             107.2 \\
           &                dialogue generation &              10 &                       2 &                   1 &               0 &                0 &             0 &                      1 &                   0 &               14 &       135.1K &              1.0 &      16.3M &               3.0 &             13.7K &              207.5 &             108.0 \\
           & knowledge-intensive language tasks &               0 &                       0 &                   0 &               0 &                2 &             0 &                      0 &                   0 &                2 &        21.8K &              1.0 &      10.7M &              64.0 &              2.7K &              465.8 &              39.3 \\
           &             question understanding &              13 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &               13 &        56.8K &              1.0 &      10.4M &              43.0 &              2.7K &              227.0 &             115.6 \\
           &              intent classification &               0 &                       6 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                6 &       149.8K &              4.8 &      10.2M &              12.0 &             591.0 &               94.2 &              53.9 \\
           &         wrong candidate generation &              14 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &               14 &        45.0K &              1.0 &       9.7M &              77.0 &              3.7K &              215.9 &             128.3 \\
           &                 question rewriting &               9 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                9 &        54.9K &              1.0 &       9.4M &              44.0 &             826.0 &              160.9 &             116.7 \\
           &                     entity linking &               0 &                       0 &                   1 &               0 &                0 &             0 &                      0 &                   0 &                1 &        18.4K &              1.0 &       9.0M &              48.0 &              2.7K &              489.4 &               0.0 \\
           &           named entity recognition &              22 &                       2 &                   0 &               0 &                0 &             0 &                      0 &                   0 &               24 &        51.0K &              1.5 &       8.4M &              13.0 &             11.9K &              133.1 &              92.0 \\
           &                  emotion detection &               0 &                       4 &                   4 &               0 &                0 &             0 &                      0 &                   0 &                8 &       188.8K &              3.4 &       7.7M &               3.0 &             363.0 &               37.9 &              19.1 \\
           &                        mathematics &               5 &                       1 &                   2 &               0 &                0 &             0 &                      0 &                   0 &                8 &        98.0K &              1.5 &       7.7M &               5.0 &             389.0 &               88.5 &              48.0 \\
           &              ethics classification &               6 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                6 &        25.3K &              1.0 &       7.5M &              69.0 &              4.1K &              355.6 &             190.0 \\
           &            language identification &              15 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &               15 &        43.2K &              1.0 &       6.6M &              32.0 &              2.8K &              182.8 &             106.0 \\
           &             question decomposition &               2 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                2 &        10.1K &              1.0 &       6.2M &             432.0 &              1.2K &              596.6 &              63.6 \\
           &               sentence compression &               1 &                       1 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                2 &       104.9K &              3.0 &       5.7M &              13.0 &             493.0 &               71.4 &              19.0 \\
           &     general language understanding &               0 &                       0 &                   0 &               0 &                0 &             5 &                      0 &                   0 &                5 &       185.3K &              1.0 &       5.6M &               7.0 &             326.0 &               33.1 &              16.5 \\
           &                text simplification &               4 &                       3 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                7 &        43.8K &              1.7 &       5.2M &              22.0 &             302.0 &              105.4 &              30.7 \\
           &                  story composition &               3 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                3 &         8.2K &              1.0 &       5.0M &             190.0 &              1.2K &              510.8 &             118.3 \\
           &                violation detection &               0 &                       1 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                1 &         9.0K &              5.0 &       4.9M &             117.0 &              3.8K &              540.4 &               0.0 \\
           &              intent identification &               4 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                4 &        18.0K &              1.0 &       4.7M &              80.0 &             982.0 &              236.3 &             111.2 \\
           &         hate speech categorization &               5 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                5 &        18.0K &              1.0 &       4.6M &             113.0 &              1.1K &              256.2 &               0.7 \\
           &                    keyword tagging &               3 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                3 &        17.0K &              1.0 &       4.5M &              50.0 &             752.0 &              227.8 &             111.2 \\
           &            euphemism understanding &               0 &                       1 &                   1 &               0 &                0 &             0 &                      0 &                   0 &                2 &        60.3K &              2.0 &       3.9M &              26.0 &             120.0 &               61.9 &              23.2 \\
           &             dialogue understanding &               0 &                       0 &                   0 &               0 &                3 &             0 &                      0 &                   0 &                3 &        55.2K &              1.0 &       3.5M &              18.0 &             878.0 &               49.1 &              30.2 \\
           &                     style transfer &               2 &                       0 &                   0 &               0 &                2 &             0 &                      0 &                   0 &                4 &        75.9K &              1.0 &       3.2M &              18.0 &             277.0 &               51.8 &              11.7 \\
           &                 social commonsense &               0 &                       1 &                   1 &               0 &                0 &             0 &                      0 &                   0 &                2 &        66.8K &              3.0 &       3.2M &              20.0 &             176.0 &               47.2 &               0.4 \\
           &                        explanation &               3 &                       0 &                   1 &               0 &                0 &             0 &                      0 &                   0 &                4 &        25.6K &              1.0 &       2.8M &              28.0 &             783.0 &              120.3 &              58.5 \\
           &                answer verification &               4 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                4 &        21.2K &              1.0 &       2.7M &              49.0 &             547.0 &              121.0 &              23.2 \\
           &            text quality evaluation &              10 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &               10 &        23.5K &              1.0 &       2.7M &              63.0 &              1.5K &              130.2 &             107.1 \\
           &             section classification &               3 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                3 &        12.0K &              1.0 &       2.5M &             165.0 &              1.2K &              313.1 &             155.8 \\
           &                  fact verification &               0 &                       2 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                2 &         4.6K &              2.0 &       2.1M &               1.0 &             890.0 &              450.8 &               2.3 \\
           &     negotiation strategy detection &               7 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                7 &         7.1K &              1.0 &       1.6M &             120.0 &             645.0 &              231.6 &              20.3 \\
           &             speaker identification &               8 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                8 &        15.2K &              1.0 &       1.6M &              52.0 &              1.4K &              218.5 &             130.1 \\
           &    funnier headline identification &               0 &                       2 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                2 &        19.0K &              7.0 &       1.5M &              37.0 &             197.0 &               79.6 &               3.1 \\
           &            grammar error detection &               2 &                       1 &                   1 &               0 &                0 &             0 &                      0 &                   0 &                4 &        28.6K &              2.0 &       1.4M &               3.0 &             150.0 &               53.1 &              37.0 \\
           &             acronym identification &               0 &                       1 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                1 &        13.8K &              6.0 &       1.4M &              23.0 &             448.0 &               99.9 &               0.0 \\
           &       word relation classification &               5 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                5 &         8.9K &              1.0 &       1.3M &              80.0 &             244.0 &              153.2 &              68.3 \\
           &                     word semantics &               9 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                9 &        19.1K &              1.0 &       1.3M &              37.0 &             248.0 &               92.4 &              49.5 \\
           &                   stance detection &               3 &                       5 &                   5 &               0 &                0 &             0 &                      0 &                   0 &               13 &        11.8K &              2.9 &       1.2M &               8.0 &             470.0 &               53.7 &              40.5 \\
           &            argument classification &               0 &                       0 &                   0 &               0 &                1 &             0 &                      0 &                   0 &                1 &        18.3K &              1.0 &       1.1M &              37.0 &             324.0 &               59.7 &               0.0 \\
           &            formal-language-to-text &               0 &                       0 &                   0 &               0 &                0 &             0 &                      2 &                   0 &                2 &        14.2K &              1.0 &       1.1M &              17.0 &             277.0 &               73.3 &              13.7 \\
           &           spelling error detection &               1 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                1 &         6.5K &              1.0 &       1.1M &             154.0 &             195.0 &              161.6 &               0.0 \\
           &                    poem generation &               1 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                1 &         6.4K &              1.0 &       1.0M &              96.0 &              3.6K &              156.4 &               0.0 \\
           &                       slot filling &               0 &                       1 &                   2 &               0 &                0 &             0 &                      0 &                   0 &                3 &        16.1K &              2.3 &     833.4K &              11.0 &             113.0 &               48.8 &               5.4 \\
           &     entity relation classification &               1 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                1 &         5.9K &              1.0 &     701.1K &             117.0 &             135.0 &              118.8 &               0.0 \\
           &         readability classification &               0 &                       1 &                   1 &               0 &                0 &             0 &                      0 &                   0 &                2 &         1.0K &              3.0 &     675.0K &             331.0 &              1.6K &              682.9 &             189.0 \\
           &                    irony detection &               2 &                       1 &                   1 &               0 &                0 &             0 &                      0 &                   0 &                4 &         8.6K &              2.0 &     586.6K &               2.0 &             341.0 &               89.3 &              59.6 \\
           &            dialogue state tracking &               2 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                2 &         4.4K &              1.0 &     478.8K &              45.0 &             564.0 &              240.5 &             145.1 \\
           &           entity linking retrieval &               0 &                       1 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                1 &        998.0 &              1.0 &     458.7K &             306.0 &             891.0 &              459.6 &               0.0 \\
           &           grammar error correction &               0 &                       1 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                1 &         4.2K &              4.0 &     428.9K &              52.0 &             256.0 &              101.6 &               0.0 \\
           &              gender classification &               1 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                1 &         6.5K &              1.0 &     354.7K &              51.0 &              60.0 &               54.6 &               0.0 \\
           &                  entity generation &               1 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                1 &         3.1K &              1.0 &     306.7K &              97.0 &             109.0 &               99.1 &               0.0 \\
           &               riddle understanding &               0 &                       1 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                1 &         3.5K &              4.0 &     211.2K &              13.0 &             585.0 &               60.2 &               0.0 \\
           &                 sentence expansion &               1 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                1 &         1.8K &              1.0 &     205.4K &              77.0 &             291.0 &              116.6 &               0.0 \\
           &                       paper review &               1 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                1 &        157.0 &              1.0 &     141.5K &             107.0 &              3.1K &              901.4 &               0.0 \\
           &                spam classification &               1 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                1 &         1.1K &              1.0 &     131.3K &             100.0 &             195.0 &              123.3 &               0.0 \\
           &       financial sentiment analysis &               0 &                       1 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                1 &         2.3K &              9.0 &     114.1K &              17.0 &             162.0 &               50.4 &               0.0 \\
           &                  number conversion &               2 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                2 &        998.0 &              1.0 &     110.0K &              54.0 &             162.0 &              110.2 &              21.4 \\
           &             preposition prediction &               1 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                1 &        926.0 &              1.0 &     102.9K &             111.0 &             115.0 &              111.2 &               0.0 \\
           &    speaker relation classification &               2 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                2 &        153.0 &              1.0 &      57.0K &             132.0 &             895.0 &              371.7 &               5.0 \\
           &               sentence composition &               3 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                3 &        462.0 &              1.0 &      51.3K &              82.0 &             179.0 &              127.9 &              28.9 \\
           &          authorship identification &               0 &                       1 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                1 &         63.0 &              6.0 &      31.3K &              83.0 &             599.0 &              496.4 &               0.0 \\
           &           coherence classification &               1 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                1 &        308.0 &              1.0 &      29.4K &              79.0 &             147.0 &               95.5 &               0.0 \\
           &        punctuation error detection &               1 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                1 &        100.0 &              1.0 &       9.1K &              74.0 &             110.0 &               91.1 &               0.0 \\
           &                            Overall &            1194 &                     195 &                 100 &              40 &               13 &            16 &                     14 &                   0 &             1572 &        43.7M &              1.7 &    5890.2M &               1.0 &            645.3K &              260.9 &             630.3 \\
    \midrule
           \multirow{10}{*}{\makecell{Valid \\ (10)}}   & cause\_effect\_classification &               7 &                       1 &                   1 &               1 &                0 &             1 &                      0 &                   0 &               11 &        17.0K &              2.3 &       2.2M &                 23 &                227 &                78.3 &               40.6 \\
           &    toxic\_language\_detection &               6 &                       1 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                7 &       106.0K &              2.4 &      10.0M &                 15 &                887 &               105.2 &                7.2 \\
           &          linguistic\_probing &               3 &                       0 &                   3 &               0 &                0 &             0 &                      0 &                   0 &                6 &        20.1K &              1.0 &       1.8M &                 17 &                143 &                57.2 &               34.1 \\
           &          question\_answering &               2 &                       2 &                   2 &               0 &                0 &             0 &                      0 &                   0 &                6 &        22.8K &              2.3 &      10.9M &                 81 &               1485 &               423.7 &              104.3 \\
           &        stereotype\_detection &               1 &                       4 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                5 &         2.0K &              5.8 &       0.1M &                 21 &                150 &                51.6 &               44.2 \\
           &           sentence\_ordering &               2 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                2 &         0.7K &              1.0 &       0.1M &                143 &                287 &               192.1 &                4.4 \\
           &         dialogue\_generation &               0 &                       0 &                   1 &               0 &                0 &             0 &                      0 &                   0 &                1 &         3.1K &              1.0 &       0.3M &                  8 &                384 &               109.0 &                0.0 \\
           &        sentence\_composition &               1 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                1 &         0.6K &              1.0 &       0.1M &                 58 &                115 &                85.2 &                0.0 \\
           &               summarization &               1 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                1 &         2.3K &              1.0 &       1.1M &                279 &               1305 &               465.7 &                0.0 \\
           &                data\_to\_text &               0 &                       0 &                   0 &               0 &                0 &             0 &                      1 &                   0 &                1 &         7.7K &              1.0 &       1.5M &                 54 &              25692 &               190.5 &                0.0 \\
           &                     Overall &              23 &                       8 &                   7 &               1 &                0 &             1 &                      1 &                   0 &               41 &       182.1K &              2.4 &      28.0M &                  8 &              25692 &               145.7 &              142.3 \\
    \midrule
            \multirow{15}{*}{\makecell{Test \\ (15)}}   &     question\_answering &              68 &                       7 &                   5 &               6 &                0 &             2 &                      0 &                   0 &               88 &       118.3K &              1.9 &         -- &                -- &                -- &                 -- &                -- \\
           &        textual\_entailment &              27 &                      21 &                   7 &               9 &                0 &            10 &                      0 &                   5 &               79 &       567.4K &              4.5 &         -- &                -- &                -- &                 -- &                -- \\
           &           text\_completion &              19 &                      11 &                   3 &               2 &                0 &             0 &                      0 &                   0 &               35 &       174.4K &              2.8 &         -- &                -- &                -- &                 -- &                -- \\
           &    coreference\_resolution &              12 &                      10 &                   3 &               4 &                0 &             3 &                      0 &                   1 &               33 &        53.5K &              3.6 &         -- &                -- &                -- &                 -- &                -- \\
           &         fact\_verification &               3 &                       5 &                   4 &               0 &                0 &             0 &                      2 &                   4 &               18 &       178.7K &              1.7 &         -- &                -- &                -- &                 -- &                -- \\
           &  toxic\_language\_detection &               4 &                       2 &                   9 &               0 &                0 &             0 &                      0 &                   0 &               15 &         8.4K &              1.5 &         -- &                -- &                -- &                 -- &                -- \\
           &              data\_to\_text &               4 &                       2 &                   1 &               3 &                0 &             0 &                      1 &                   3 &               14 &        64.6K &              3.1 &         -- &                -- &                -- &                 -- &                -- \\
           &  dialogue\_act\_recognition &               7 &                       1 &                   0 &               0 &                1 &             0 &                      1 &                   1 &               11 &        33.4K &              1.3 &         -- &                -- &                -- &                 -- &                -- \\
           &      stereotype\_detection &               7 &                       2 &                   1 &               0 &                0 &             1 &                      0 &                   0 &               11 &        19.9K &              1.8 &         -- &                -- &                -- &                 -- &                -- \\
           &              word\_analogy &               8 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   1 &                9 &         7.7K &              1.0 &         -- &                -- &                -- &                 -- &                -- \\
           &             summarization &               1 &                       1 &                   1 &               1 &                0 &             0 &                      0 &                   1 &                5 &        40.7K &              4.2 &         -- &                -- &                -- &                 -- &                -- \\
           & word\_sense\_disambiguation &               0 &                       1 &                   1 &               1 &                0 &             1 &                      0 &                   1 &                5 &         4.1K &              4.6 &         -- &                -- &                -- &                 -- &                -- \\
           &        overlap\_extraction &               2 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   1 &                3 &        19.2K &              1.0 &         -- &                -- &                -- &                 -- &                -- \\
           &  grammar\_error\_correction &               2 &                       1 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                3 &         8.0K &              3.0 &         -- &                -- &                -- &                 -- &                -- \\
           &       dialogue\_generation &               1 &                       0 &                   0 &               0 &                0 &             0 &                      0 &                   0 &                1 &         0.2K &              1.0 &         -- &                -- &                -- &                 -- &                -- \\
           &                   Overall &             165 &                      64 &                  35 &              26 &                1 &            17 &                      4 &                  18 &              330 &      1298.4K &              2.8 &         -- &                -- &                -- &                 -- &                -- \\
    \bottomrule
    \caption{Task split details}
    \label{tab:task_split_details}
\end{longtable}
}
\end{landscape}
